DrivingGPT: Unifying Driving World Modeling and Planning with Multi-modal Autoregressive Transformers

World model-based searching and planning are widely recognized as a promising path toward human-level physical intelligence. However, current driving world models primarily rely on video diffusion models, which specialize in visual generation but lack the flexibility to incorporate other modalities like action. In contrast, autoregressive transformers have demonstrated exceptional capability in modeling multimodal data. Our work aims to unify both driving model simulation and trajectory planning into a single sequence modeling problem. We introduce a multimodal driving language based on interleaved image and action tokens, and develop DrivingGPT to learn joint world modeling and planning through standard next-token prediction. Our DrivingGPT demonstrates strong performance in both action-conditioned video generation and end-to-end planning, outperforming strong baselines on large-scale nuPlan and NAVSIM benchmarks.

==> figures/action_distribution.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=1.0\linewidth]{example-image-a}
    \caption{action distribution.}
    \label{fig:distribution}
\end{figure}

==> tables/1-vae_ablation.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{ccccccc}
        \toprule
        ratio & img size & token length & rFID$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
        \midrule
        \multirow{3}{*}{16} & 288$\times$512 & 576   & - & - & - & - \\
                            & 432$\times$768 & 1296  & - & - & - & - \\
                            & 576$\times$1024 & 2304 & - & - & - & - \\
        \midrule
        \multirow{2}{*}{8}  & 288$\times$512 & 2304  & - & - & - & - \\
                            & 432$\times$768 & 5184  & - & - & - & - \\
        \bottomrule
    \end{tabular}
    \caption{Table showing image size, token size, and performance metrics for different ratios, including LPIPS.}
\end{table*}

==> tables/2-video_gen_quality.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{lllccc}
\toprule
\textbf{Category} & \textbf{Type} & \textbf{Model} & \textbf{\#Para.} & \textbf{FID$\downarrow$} & \textbf{FVD$\downarrow$} \\
\midrule
\multirow{9}{*}{Surround View} 
& \multirow{3}{*}{GAN} & BigGAN & 112M & --- & --- \\
& & GigaGAN & 569M & --- & --- \\
& & StyleGAN-XL & 166M & --- & --- \\
\cmidrule{2-6}
& \multirow{4}{*}{Diffusion} & ADM & 554M & --- & --- \\
& & CDM & --- & --- & --- \\
& & LDM-4 & 400M & --- & --- \\
& & DiT-XL/2 & 675M & --- & --- \\
\cmidrule{2-6}
& \multirow{2}{*}{Mask.} & MaskGIT & 227M & --- & --- \\
& & MaskGIT-re & 227M & --- & --- \\
\midrule
\multirow{15}{*}{Front View} 
& \multirow{7}{*}{AR} & VQGAN & 227M & --- & --- \\
& & VQGAN & 1.4B & --- & --- \\
& & VQGAN-re & 1.4B & --- & --- \\
& & ViT-VQGAN & 1.7B & --- & --- \\
& & ViT-VQGAN-re & 1.7B & --- & --- \\
& & RQTran. & 3.8B & --- & --- \\
& & RQTran.-re & 3.8B & --- & --- \\
\cmidrule{2-6}
& \multirow{8}{*}{AR} & LlamaGen-B (cfg=2.00) & 111M & --- & --- \\
& & LlamaGen-L (cfg=2.00) & 343M & --- & --- \\
& & LlamaGen-XL (cfg=1.75) & 775M & --- & --- \\
& & LlamaGen-XXL (cfg=1.75) & 1.4B & --- & --- \\
& & LlamaGen-3B (cfg=1.65) & 3.1B & --- & --- \\
& & LlamaGen-3B (cfg=1.75) & 3.1B & --- & --- \\
& & LlamaGen-3B (cfg=2.00) & 3.1B & --- & --- \\
\bottomrule
\end{tabular}
\caption{Performance comparison of various video world models on nuScenes. FID (Fréchet Inception Distance) and FVD (Fréchet Video Distance) are standard metrics for generation quality.}
\end{table*}

==> tables/3-extra_video_gen_metric_and_dataset.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{llccc}
\toprule
\textbf{Dataset} & \textbf{Model} & \textbf{\#Para.} & \textbf{FID$\downarrow$} & \textbf{FVD$\downarrow$} \\
\midrule
\multirow{4}{*}{NAVSIM} 
 & SVD w/o finetune & 2.5B & 27.80 & 483.76 \\
 & SVD w/ finetune & 2.5B & 25.85 & 244.31 \\
 & DriveWM GPT w/ VQ Decoder & 166M & --- & --- \\
 & DriveWM GPT w/ SVD Decoder & 166M & --- & --- \\
\midrule
\multirow{4}{*}{DrivingDojo} 
 & SVD w/o finetune & 112M & --- & --- \\
 & SVD w/ finetune & 569M & --- & --- \\
 & DriveWM GPT w/ VQ Decoder & 166M & --- & --- \\
 & DriveWM GPT w/ SVD Decoder & 166M & --- & --- \\
\bottomrule
\end{tabular}
\caption{Performance comparison of various generative models. FID (Fréchet Inception Distance) and FVD (Fréchet Video Distance) are standard metrics for generation quality. }
\end{table*}

==> tables/4-action_instruction_following.tex <==
\begin{table*}[htbp]
\centering
\caption{\textbf{Action instruction following on the DrivingDojo dataset}. $^*$  denotes the model is applied zero-shot to this dataset without fine-tuning.}
\label{tab:exp_action}
\begin{tabular}{c|c|cc|cc}
\toprule
Action Type & Test Dataset& FID & FVD & $E^{\text{AIF}}_x$($\downarrow$) & $E^{\text{AIF}}_y$($\downarrow$) \\
\midrule
In-Domain & DrivingDojo & 37.07 & 658.72 & 0.068m & 0.060m \\
Out-of-Domain & DrivingDojo & 38.30 & 716.44 & 0.133m & 0.099m  \\
\midrule
Out-of-Domain & OpenDV-2K$^*$& 24.27& 442.67 & 0.175m & 0.121m\\
\bottomrule
\end{tabular}
\end{table*}

==> tables/6-planning_results_navsim.tex <==
\begin{table}[ht]
\centering
\scriptsize
\caption{NavSim Benchmark. We show the no at-fault collision (NC), drivable area compliance (DAC), time-to-collision (TTC), comfort (Comf.), and ego progress (EP) subscores, and the PDM Score (PDMS), as percentages. Relying on the ego status is insufficient for competitive results. While sensor agents improve, the gap to human performance highlights our benchmark’s challenges.}
\begin{tabular}{l|cccc|cc|ccc|c}
\toprule
\textbf{Method} & \textbf{Ego Stat.} & \textbf{Image} & \textbf{LiDAR} & \textbf{Video} & \textbf{NC $\uparrow$} & \textbf{DAC $\uparrow$} & \textbf{TTC $\uparrow$} & \textbf{Comf. $\uparrow$} & \textbf{EP $\uparrow$} & \textbf{PDMS $\uparrow$} \\ 
\hline
Constant Velocity & \checkmark & & & & 69.9  & 58.8   & 49.3   & 100 & 49.3   & 21.6  \\ 
Ego Status MLP   & \checkmark    & & & & 93.0  & 77.3   & 83.6   & 100    & 62.8   & 65.6  \\ 
\hline
LTF & \checkmark    & \checkmark  & \checkmark  & & 97.4  & \textbf{92.8}    & 92.4   & 100    & 79.0   & 83.8  \\ 
TransFuser   & \checkmark    & \checkmark  & & \checkmark  & 97.7  & \textbf{92.8}    & 92.9   & 100    & 79.2   & \textbf{84.0}   \\ 
UniAD   & \checkmark    & \checkmark  & & \checkmark  & 97.8  & 91.9   & 92.9   & 100    & 78.8   & 83.4  \\ 
PARA-Drive   & \checkmark    & \checkmark  & \checkmark  & & \textbf{97.9}   & 92.4   & \textbf{93.0}    & 99.8   & 79.3   & \textbf{84.0}   \\ 
PARA-Drive   & \checkmark    & \checkmark  & \checkmark  & & \textbf{97.9}   & 92.4   & \textbf{93.0}    & 99.8   & 79.3   & \textbf{84.0}   \\ 
\bottomrule
\end{tabular}
\end{table}

==> tables/model_size.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{cccc}
        \toprule
        Parameters &  FVD$\downarrow$ & FID$\downarrow$ & CE Loss(train)$\downarrow$\\
        \midrule
        100M &  170.19 & 13.47 & 3.6\\
        300M &  164.42 & 13.18 & 3.2\\
        1.4B &  155.60 & 13.05 & 2.4 \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Comparison of different model sizes.}}
    \label{tab:model_size}
\end{table}
